Crystal: Introspective Reasoners Reinforced with Self-Feedback

Extensive work has shown that the performance and interpretability of commonsense reasoning can be improved via knowledge-augmented reasoning methods, where the knowledge that underpins the reasoning process is explicitly verbalized and utilized. However, existing implementations, including "chain-of-thought" and its variants, fall short in capturing the introspective nature of knowledge required in commonsense reasoning, and in accounting for the mutual adaptation between the generation and utilization of knowledge. We propose a novel method to develop an introspective commonsense reasoner, Crystal. To tackle commonsense problems, it first introspects for knowledge statements related to the given question, and subsequently makes an informed prediction that is grounded in the previously introspected knowledge. The knowledge introspection and knowledge-grounded reasoning modes of the model are tuned via reinforcement learning to mutually adapt, where the reward derives from the feedback given by the model itself. Experiments show that Crystal significantly outperforms both the standard supervised finetuning and chain-of-thought distilled methods, and enhances the transparency of the commonsense reasoning process. Our work ultimately validates the feasibility and potential of reinforcing a neural model with self-feedback.

==> floats/ablations.tex <==
\begin{table}[t]
\setlength{\tabcolsep}{2pt}
\begin{minipage}{0.52 \linewidth}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{ll ccccc ccccc ccccc c}
\toprule
\textbf{Method} & \textbf{Size} & \textbf{Seen} \\
\midrule
\methodname{} (ours) & 770M & \textbf{66.74} \\
\quad - Stage II & 770M & 66.16 \\
\qquad + Direct QA loss & 770M & 65.36 \\
\midrule
\methodname{} (ours) & 3B & \textbf{78.33} \\
\quad - Stage II & 3B & 77.79 \\
\midrule
\methodname{} (ours) & 11B & \textbf{84.58} \\
\quad - Stage II & 11B & 84.08 \\
\bottomrule
\end{tabular}
}%
\end{minipage}
\hfill
\begin{minipage}{0.46 \linewidth}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccc}
\toprule
\textbf{Stage I} & \textbf{Stage II} & \textbf{Seen} \\
\midrule
interleaved & interleaved & \textbf{66.74} \\
joint & interleaved & 66.66 \\
joint & joint & 66.31 \\
\bottomrule
\end{tabular}
}%
\end{minipage}
\caption{
    \textbf{Left:} Ablations on the RL training stage (i.e., stage II).
    Average accuracy on the development set of seen datasets is reported.
    \minor{(- Stage II is ImitationQA-v3.9.0.1, v3.12.1, v3.12.2)}
    \textbf{Right:} Ablations on the interleaved training objectives.
    Average accuracy on the development set of seen datasets is reported.
    \minor{(joint-interleaved is RainierQA-v3.11.2; joint-joint is RainierQA-v3.11.3)}
}
\label{tab:ablations}
\end{table}

==> floats/trash/function.tex <==
\begin{figure*}[!h]
\centering
\begin{minipage}{0.32 \textwidth}
\includegraphics[width=\textwidth]{images/Screenshot 2023-05-08 at 12.23.36.png}
\end{minipage}
\hfill
\begin{minipage}{0.32 \textwidth}
\includegraphics[width=\textwidth]{images/Screenshot 2023-05-08 at 12.23.45.png}
\end{minipage}
\hfill
\begin{minipage}{0.32 \textwidth}
\includegraphics[width=\textwidth]{images/Screenshot 2023-05-18 at 10.29.14.png}
\end{minipage}
\caption{
    Comparing the workflow of a vanilla QA model (left), Rainier (middle), and \methodname{} (right).
}
\label{fig:function}
% \vspace{-16pt}
\end{figure*}

==> sections/ethics.tex <==
\section*{Ethics Statement}
\label{sec:ethics}

==> sections/method.tex <==
\section{Method}
\label{sec:method}

% \input{floats/function}

% In this section, 
We will first introduce some background on knowledge introspection and RL (\S\ref{sec:background}), followed by our introspective reasoning model, including its basic functionality (\S\ref{sec:introspective_reasoning}), the input/output format (\S\ref{sec:format}), the implications of our model on the RL algorithm (\S\ref{sec:model_sharing}), and the design of model training process (\S\ref{sec:two_stage}, \S\ref{sec:interleave}).

\subsection{Background: Knowledge Introspection, Reinforcement Learning  (RL), PPO}
\label{sec:background}

\paragraph{Knowledge introspection.}
Knowledge introspection is the process of generating knowledge statements that are relevant to the reasoning on a question \citep{Liu2021GeneratedKP, Liu2022RainierRK}.
The goal is to produce knowledge statements that are useful in prompting a downstream QA model to make more accurate predictions, while making the problem-solving process more interpretable by exposing the knowledge that constitutes the reasoning chains.
For example, given the question \textit{``What comes from cows?''} with the correct answer \textit{``nutritious fluids''} given among other incorrect choices, the knowledge introspector may generate knowledge statements like \textit{``Cows produce milk.''}
Taking this knowledge statement as additional input, a QA model becomes more likely to predict the correct answer.
Conceptually, knowledge introspection is performed by a generative language model $p(k | q; \theta)$ that takes a question $q$ as input and generates a knowledge statement $k$.

% \paragraph{\exmethodname{}, a reinforced knowledge introspector.}
\paragraph{\exmethodname{} and RL.}
\citet{Liu2022RainierRK} developed a knowledge introspection model called \textbf{\exmethodname{}}.
To solve commonsense problems, \exmethodname{} is complemented by generic QA models like \textsc{UnifiedQA} \citep{Khashabi2020UnifiedQACF}, \dif{which is a sequence-to-sequence model that generates an answer for a given question accompanied by an optional context.} % \asli{may need to explain UnifiedQA a bit since we refer to it in the experiments}
% \exmethodname{} \citep{Liu2022RainierRK} is a dedicated model for knowledge introspection.
% It focuses on generating commonsense knowledge related to a question, and does not have a knowledge-grounded reasoning mode that predicts answers.
% When \exmethodname{} is used in practice, knowledge-grounded reasoning is delegated to an existing QA model such as \model{UnifiedQA} \citep{Khashabi2020UnifiedQACF}.
% Compared with \exmethodname{}, \methodname{} does both knowledge introspection and knowledge-grounded reasoning, and is thus a self-contained model for solving commonsense QA problems.
% \paragraph{Reinforcement Learning, PPO.}
\exmethodname{} is trained using RL.
This is because there are usually no gold knowledge labels as supervision for the knowledge introspector.
Concurrently, the efficacy of the generated knowledge statements can be assessed based on their impact on the QA model.
Specifically, a reward function is designed to determine of prompting the QA model with the knowledge statement can correct an otherwise faulty prediction.
The training objective of \exmethodname{} is to maximize this reward, with the QA model remaining fixed throughout this process. 
% This can be captured by a reward function to optimize.
Since knowledge statements are sequences of discrete tokens, knowledge generation is viewed as a sequential decision making process over the natural language vocabulary space, and an RL algorithm called Proximal Policy Optimization (PPO) \citep{Schulman2017ProximalPO} is employed to optimize the reward.
\exmethodname{} has shown to generate predominantly factual knowledge statements that are relevant to questions, significantly improving the performance of downstream QA models.

\paragraph{Proximal Policy Optimization (PPO).}
PPO \citep{Schulman2017ProximalPO} is an RL algorithm that has been widely used in aligning LMs with human feedback \citep{Stiennon2020LearningTS, Ouyang2022TrainingLM, chatgptblog}.
\citet{Liu2022RainierRK} adapts PPO to train \exmethodname{}.
Within the context of PPO terminology, the knowledge introspector assumes the role of the \textit{policy model}, while the QA model functions as the \textit{reward model}.
PPO further employs a \textit{value model} to estimate the value function for states containing partial knowledge statements.
The overall PPO loss is a combination of a policy loss and a value loss.
% Explain these? --
% KL penalty term, initial policy
% value function, value model
% PPO loss, policy loss, value loss
% lagging policy

\subsection{Introspective Reasoning Models}
\label{sec:introspective_reasoning}

Conventionally, commonsense QA models are designed to predict answers for questions \citep{Lourie2021UNICORNOR}.
We introduce \textbf{introspective reasoning models} that initially engage in introspection for commonsense knowledge related to the question, subsequently grounding their prediction in this knowledge.
The process of knowledge introspection and grounding is conducted explicitly, requiring the model to articulate the introspected knowledge as natural language statements.
Essentially, an introspective reasoning model fuses the functionalities of both the knowledge introspector and the QA model.
% We refer to such models as \textit{introspective reasoning models}.
We refer to the introspective reasoning model developed this study as \methodname{}.

\methodname{} has two modes of operation: \textit{knowledge introspection} and \textit{knowledge-grounded reasoning.}
During knowledge introspection, it accepts a question as input, and generates knowledge statement relevant to the question. This statement potentially provides evidence to either support or contradict a potential answer, forming a reasoning path towards the prediction.
In knowledge-grounded reasoning, the model ingests both the question and the knowledge statements generated during knowledge introspection as inputs. It then formulates and aggregated prediction by consulting all the available reasoning paths, effectively harnessing the power of ensembled reasoning. 

\subsection{Redesigned QA Formatting for a Multi-Mode Model}
\label{sec:format}

\input{floats/format}

Since \methodname{} has two modes of operation, it needs to discern when to conduct knowledge introspection and when to engage in knowledge-grounded reasoning.
Drawing inspiration from the work of \citet{Tafjord2021GeneralPurposeQW}, we structure the input and output format as demonstrated in \autoref{tab:format}.
% In the knowledge introspection mode, the input and output resemble the following:
% \begin{align*}
% & \texttt{\small \textcolor{red}{(Input)}} \\
% & \texttt{\small What would someone wear to protect themselves from a cannon? \textbackslash{}n} \\
% & \texttt{\small (A) ungulate (B) bomber (C) body armor (D) tank (E) hat \textbackslash{}n} \\
% & \texttt{\small Knowledge:} \\
% & \texttt{\small \textcolor{red}{(Output)}} \\
% & \texttt{\small Tanks can fire bombs.}
% \end{align*}
% In the knowledge-grounded reasoning mode, the input and output resemble the following:
% \begin{align*}
% & \texttt{\small \textcolor{red}{(Input)}} \\
% & \texttt{\small What would someone wear to protect themselves from a cannon? \textbackslash{}n} \\
% & \texttt{\small (A) ungulate (B) bomber (C) body armor (D) tank (E) hat \textbackslash{}n} \\
% & \texttt{\small Knowledge: Tanks can fire bombs. \textbackslash{}n} \\
% & \texttt{\small Answer:} \\
% & \texttt{\small \textcolor{red}{(Output)}} \\
% & \texttt{\small D}
% \end{align*}
This format is adapted from \textsc{UnifiedQA} \citep{Khashabi2020UnifiedQACF}, based on which we made the following changes:
\begin{itemize}\itemsep0em 
\item The input is appended with a marker that indicates which mode of operation is desired. In knowledge introspection this marker is \texttt{``Knowledge:''}, and in knowledge-grounded reasoning it is \texttt{``Answer:''}.
\item The output is the letter for the predicted answer choice, not the actual content of an answer choice.
\item The input and output text are not lowercased.
\end{itemize}

\subsection{Model Sharing in PPO}
\label{sec:model_sharing}

% \paragraph{Model sharing.}
% \ram{make these three paragraphs as sub-paras of "Space and time complexity of METHODNAME?" or something along those lines.} \gary{Agreed, while I think the model sharing paragraph belongs to this section.}
Following \exmethodname{}, we utilize PPO algorithm to train \methodname{}. 
Since \methodname{} combines the functionalities of both the knowledge introspector and the QA model, it serves as both the policy model and the reward model during PPO training.
% : the policy model is \methodname{} used under the knowledge introspection mode, and the reward model is \methodname{} used under the knowledge-grounded reasoning mode.
Moreover, we propose to repurpose \methodname{} as the value model, resulting in the same underlying model being used for policy, value, and reward.
% Therefore, we use the same underlying model across policy, value and reward.
\methodname{} is essentially a generative LM equipped with two heads: a LM head, which comes into play during the policy and reward modeling, and a value regression head, activated during the value modeling process. 
% (which is active when modeling the value).
% \todo{Add a schematic figure for the model architecture.}

\subsection{Two-Staged Training}
\label{sec:two_stage}

PPO requires that the policy model is initialized from a reasonably good state.
Typically, PPO training follows a supervised finetuning stage for the policy model \citep{Stiennon2020LearningTS, Ouyang2022TrainingLM}.
\dif{For \exmethodname{}, an imitation learning stage, during which the model is supervised on knowledge statements obtained from a few-shot \model{GPT-3} knowledge introspector (i.e., \textit{silver knowledge labels}), precedes the RL training stage.}
This imitation learning stage imparts the model with the basic functionality of generating question-specific knowledge, and sets a promising starting point for RL.
% \asli{need to explicitly define what 'silver' means here, you use in the experiments as well. }

Drawing from this concept, we also implement a two-stage training process for \methodname{}.
In training stage I, the model is trained to carry out both knowledge introspection (by imitating a few-shot \model{GPT-3} knowledge introspector) and knowledge-grounded reasoning.
We minimize two losses: a knowledge introspection loss % (a.k.a., $Q \rightarrow K$ loss)
\begin{align*}
\loss_\text{QK}(\theta) &= -\log{p_\text{QK}(k | q; \theta)},
\end{align*}
and a knowledge-grounded reasoning loss % (a.k.a., $Q + K \rightarrow A$ loss)
\begin{align*}
\loss_\text{QKA}(\theta) &= -\log{p_\text{QKA}}(a^* | q, k; \theta),
\end{align*}
where $q$ is the question (including choices), $a^*$ is the correct answer label, and $k$ is a knowledge statement generated by the few-shot \model{GPT-3}.
The \methodname{} model is parameterized by $\theta$.
$p_\text{QK}(\cdot; \theta)$ denotes the language modeling probability in the knowledge introspection mode, and $p_\text{QKA}(\cdot; \theta)$ denotes the language modeling probability in the knowledge-grounded reasoning mode.

In training stage II, we use RL to optimize the knowledge introspection mode, while maintaining the same supervised loss to fine-tune the knowledge-grounded reasoning mode.
This involves minimizing two distinct losses: a knowledge introspection loss $\loss_\text{PPO}(\theta)$, and a knowledge-grounded reasoning loss:
\begin{align*}
\loss_\text{QKA}(\theta) &= -\log{p_\text{QKA}}(a^* | q, k; \theta),
\end{align*}
where $k \sim p_\text{QK}(\cdot | q; \theta)$ is sampled on-policy from \methodname{}.

\input{floats/interleave}

\subsection{Interleaved Objectives}
\label{sec:interleave}

Through empirical analysis, we have observed interleaving the to training losses in each stage yields beneficial outcomes as opposed to jointly optimizing them.
In stage I, we optimize $\loss_\text{QK}$ for a specific number of iterations, followed by optimizing $\loss_\text{QKA}$ for another set number of iterations, repeating this cycle.
Similarly, In stage II, we optimize $\loss_\text{PPO}$ for a designated number of iterations, followed by optimizing $\loss_\text{QKA}$ for another set number of iterations, repeating this cycle.
This design bears resemblance to the EM algorithm \citep{dempster1977maximum}, wherein the hidden variable corresponds to the knowledge statement. Optimizing $\loss_\text{PPO}$ can be likened to estimating the hidden variables, while optimizing $\loss_\text{QKA}$ is akin to updating the parameter estimation based on the current assignment of hidden variables. % \gary{Maybe this is a bad analogy, let me know if this is inappropriate and I will remove this.} \asli{i actually like this analogy, revised it.}
The interleaved training process is illustrated in \autoref{fig:interleave}.

% The model sharing in PPO implies that the reward model will inevitably become dynamic over the course of training.
% This means solely minimizing the PPO loss, $\loss_\text{PPO}$, can destructively interfere with \methodname{}'s capability to do knowledge-grounded reasoning.
% We need to maintain this operation mode by introducing an auxiliary training loss during RL:
% \begin{align*}
% \loss_\text{QKA} = -\log{p_\theta(a \mid q \circ k)}
% \end{align*}
% Empirically, we found that it is most beneficial to interleave $\loss_\text{PPO}$ and $\loss_\text{QKA}$ at a certain cadence, that is, optimize $\loss_\text{PPO}$ for some number of iterations, and then optimize $\loss_\text{QKA}$ for some number of iterations, and repeat this cycle.

